Natural Language Processing for Systems Engineering: Automatic Generation of Systems Modelling Language Diagrams

The design of complex engineering systems is an often long and articulated process that highly relies on engineers' expertise and professional judgment. As such, the typical pitfalls of activities involving the human factor often manifest themselves in terms of lack of completeness or exhaustiveness of the analysis, inconsistencies across design choices or documentation, as well as an implicit degree of subjectivity. An approach is proposed to assist systems engineers in the automatic generation of systems diagrams from unstructured natural language text. Natural Language Processing (NLP) techniques are used to extract entities and their relationships from textual resources (e.g., specifications, manuals, technical reports, maintenance reports) available within an organisation, and convert them into Systems Modelling Language (SysML) diagrams, with particular focus on structure and requirement diagrams. The intention is to provide the users with a more standardised, comprehensive and automated starting point onto which subsequently refine and adapt the diagrams according to their needs. The proposed approach is flexible and open-domain. It consists of six steps which leverage open-access tools, and it leads to an automatic generation of SysML diagrams without intermediate modelling requirement, but through the specification of a set of parameters by the user. The applicability and benefits of the proposed approach are shown through six case studies having different textual sources as inputs, and benchmarked against manually defined diagram elements.

==> graveyard.tex <==
% The selected key phrases and relationships are then mapped to SysML model elements and augmented in subsequent steps for plotting SysML diagrams. 

% Tf-idf calculates a relative weighting for each word in a document according to its frequency in the document and its relative commonness across the corpus. 

%Additionally, one phrase is selected from each document as the parent phrase for clearer diagram plotting, and the phrases are listed in Table~\ref{table:datasets}. The use of these phrases is explained in Section~\ref{section:successdiagramgeneration}.

%The results are validated against manually constructed diagrams. The performance of each step in the approach is first evaluated, to then quantify the overall effectiveness of the approach in automatic SysML diagram generation. 


%Additionally, the key textual relationships need to be further classified using a set of heuristics rules and used to generate different SysML relationships. In this process, the list of textual relationships and phrases are also augmented to make the resultant diagrams more complete.

%The corpus can be enriched by including other text documents that belong to similar domains. For example, when investigating the dependencies between components of a passenger car, if only 100 text documents are available, additional documents on sports cars and trucks could be included in the corpus. In constructing the SysML diagram, the user would need to select a subset of documents from the input corpus to plot the SysML diagrams. 


% why is this importnat ? "and a relationship is considered a key relationship if it connects two key entities. "


% note: the equation MUST BE REWRITTEN

%Semantic relationships such as hypernyms/hyponyms between individual synsets are stored in the WordNet and can be retrieved easily. However, each word may be assigned different synsets because of polysemy. Thus, in this study, a word sense disambiguation algorithm, 

% you have to explain each term briefly and clearly. 

% this part is very unclear. Given that each entity has to word, are you considering the tf-idf of each word and then taking the average of the two? if so, please be very clear about it. If not, please explain.

% similarly when using the entity frequency, you need to define it. Does it mean that you are counting the frequency of the subject-object entity within the corpus? Or within a document? Please, be very specfic about it.

% The Wordnet depth of information refers to ????? 
% again, very unclear what is meant.
 
% Not clear at all what was meant by this phrase or by this equation. `This study proposed the following formula to score each subject and object entity that are outputs of the previous step. ' I would rewrite it to:

% this phrase is unclear and useless is put at the end. Please please please, make everything clearer "This formula takes into account the domain relevance of the entity using the tf-idf value of each term in the entity. It also considers the frequency of each entity to evaluate the significance of the entity. Semantic meaning is also taken into account using the WordNet depth measure. "

%YOU NEED TO have a section with A LIST OF steps (bullet points) of  WHAT THE USER NEEDS TO DO:

%1. Select dataset - btw why 2 documents below?
%2. Set treshold values for ££££ be very specific here
%3. ....

%Note: these steps should map exactly the subsections that you have in section 4


% this section was not useful here. text has been moved where more appropriate. Please check the difference

% \subsection{Evaluation Procedure}
% The performance of each step in the approach is first evaluated, to then quantify the overall effectiveness of the approach in automatic SysML diagram generation. 

% the phrase that follows does not belong to the applications, IT MUST BE MOVED TO THE 3.7 SECTION     As the aim of the approach is not to replace systems engineers but rather to aid them in gaining an overview of the system, the goal is not a perfect extraction of nouns or relationships. Rather, it is to provide an overview of the selected document and system through the profiles in SysML diagrams. Thus, the results are evaluated against manually constructed benchmarks. 


% if wordnet was so important to be indicated almost immediately in the conclusions, why doesn't it appear in the abstract and in the introduction?? 
%Just expand a bit more this first paragraph

Moreover, systems engineers will be able to amend potential oversights in the diagrams generated by offering suggestions through augmented entities. 

% Too many details. 
% For future work, the authors suggest extending to additional SysML diagrams. Obvious candidates are package diagrams and use case diagrams, which can be easily extracted based on the abstractions and requirements that are already generated in this algorithm. Additionally, to demonstrate the proposed approach, this study has used mostly simple off-the-shelf techniques in extracting entities and relationships and plotting diagrams. It would also be useful to research into employing more sophisticated and customised techniques for keyword extraction, relationship extraction, and graphical layouts algorithm to suit SysML diagrams better.  


% consider discussing the effect of shorter texts/smaller number of documents
% consider including a study of the effect of different parameters?
% relate back to claims made in the introduction


%To fully evaluate the proposed approach in selecting key entities, the threshold for tf-idf value $\sigma_{tf-idf}$ is set as zero in the case studies. However, it is envisioned that it can be adjusted according to the user’s needs. Additionally, the threshold for the likelihood of a valid relation $\sigma_{relationship}$ is set as 0.5. The OpenIE toolbox attempts to extract multiple relations for every sentence, thus the threshold is set at 0.5 to remove an excessive number of duplicated relationships. The threshold for key entities $\sigma_{entity}$ is set at 0.1 and the threshold for classifying composite relationships $\sigma_{rel difference}$ is set at 0.2. The specificity of entities $L_{entity}$ is set at 3. 

% I do not think you have introduced all the hyperparameters in the main body of the manuscript. Please revised this and be more direct on explaining why you set some. YOU MUST USE THE SAME LANGUAGE AND NOTATION USED BEFORE

 
% note the change: subject/object to subject-object
% There might have been a confusion here. The subject and object could be phrases. Each subject phrase and each object phrase are considered entities by themselves. 
 
% which can vary across different runs according to the needs of the user. Importantly


% requirement generation, specification, refer to friedenthal14practical book
Typical systems engineering methods, tools or frameworks include graphical modelling languages~\cite{friedenthal14practical,delligatti2013sysml,huang2007system}, design models~\cite{hart2015introduction}, lifecycle models~\cite{friedenthal14practical}, etc, that aid system engineers in designing complex systems. 

Blocks are basic structural elements of SysML \cite{friedenthal14practical,omg19omg,friedenthal08omg,hause06thesysml}. They could represent the types of components in the system, definitions of components, or requirements \cite{friedenthal14practical,omg19omg,friedenthal08omg,hause06thesysml}. In this study, blocks are assumed be defined by noun phrases that are explicitly written in the documents. Thus, t

Relationships between blocks form another element of SysML diagrams \cite{friedenthal14practical,omg19omg,friedenthal08omg,hause06thesysml}. SysML contains many relationship categories for different diagrams, for example generalisations and dependencies for structure diagrams, and containment and trace for requirement diagrams \cite{friedenthal14practical,omg19omg,friedenthal08omg,hause06thesysml}. 
